Software Engineers Response to Public Crisis: Lessons Learnt from Spontaneously Building an Informative COVID-19 Dashboard

The Coronavirus disease 2019 (COVID-19) outbreak quickly spread around the world, resulting in over 240 million infections and 4 million deaths by Oct 2021. While the virus is spreading from person to person silently, fear has also been spreading around the globe. The COVID-19 information from the Australian Government is convincing but not timely or detailed, and there is much information on social networks with both facts and rumors. As software engineers, we have spontaneously and rapidly constructed a COVID-19 information dashboard aggregating reliable information semi-automatically checked from different sources for providing one-stop information sharing site about the latest status in Australia. Inspired by the John Hopkins University COVID-19 Map, our dashboard contains the case statistics, case distribution, government policy, latest news, with interactive visualization. In this paper, we present a participant's in-person observations in which the authors acted as founders of https://covid-19-au.com/ serving more than 830K users with 14M page views since March 2020. According to our first-hand experience, we summarize 9 lessons for developers, researchers and instructors. These lessons may inspire the development, research and teaching in software engineer aspects for coping with similar public crises in the future.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we discuss some observation of other data sources when developing our dashboard, and we also introduce the implications behind our project.

% \subsection{Issues with the Government Report}
% %Another thing that caught our attention is that government information disclosure work has some room to improve. During the two months of collecting data from all levels of Australian state government websites, we found out four types of problems that keep occurring, which confused and anxious the audience:
% The daily report about COVID-19 from Government is the most important data resource of our site.
% However, during the two-month data collection, we witness several issues of it: 
% \begin{itemize}
%     \item \textbf{Data inconsistency:} Australia is a federated commonwealth, and as such, each state may adopt different standards to release the data. The confirmed cases of some states reflect where the person usually lives, while other states report new cases based on where patients were tested. Such inconsistency confuses users and also make their reports less convincing to the public.
%     %The data inconsistent between the state government report and the federal government report has happened in several states. It can be confused to us during the data collection and also to the public users as they do not know which number is correct. If we use the federal government report, then users would leave feedback like our data is not the same with what they saw on the state government and vice versa.
%     \item \textbf{Uncertainty of update time:} State Government websites may release their daily reports about COVID-19 anytime from early morning to late evening. Some data like test number may not be updated for several days. Such uncertainty may make the public more anxious about the unknown situation.
%      % For some state, sometimes they release their update in the morning and sometimes in the evening. Users are not satisfied with this uncertainty of the update time. 
%     \item \textbf{Not Mobile Friendly:} With the popularity of mobile devices, most users begin to use mobile phones to access the information. However, most Government websites especially the rich data are not mobile friendly.
%     %Based on our Google Analytics Report, most of the users are using mobile devices. However, the system or the framework government websites are using, are not mobile-friendly, and some of the dashboards are just a static pdf file, which does not allow users to interact with. 
%     %\item \textbf{Format is frequently changing while the update time is too long:} The state government websites tried to keep updating to provide a better service to the public, which is a good thing. However, the changes they have made were too different from the previous one, which is a lack of design consistency. Moreover, the update time takes too long, sometimes, it takes 1-2 days to update, and the public cannot access the dashboard during the update. This could make users anxious about the unknown situation.
% \end{itemize}

% We hope that these observations may raise the attention of the Government for reflecting their information display.
% They can further improve their sites by lessons learned about data visualization and web development during our dashboard development.

% \subsection{Implication about the Extension}
% Although we are developing the information dashboard for COVID-19, it can be extended to other crises such as the seasonal flu, bush fire, flood, locust plague, and some other sorts of infectious diseases. 
% During the development of this dashboard, we try to abstract a template including a set of crawlers with a mechanism of involving human in the loop as the backend, and data visualization for different kinds of data on the front end.
% All other functionalities such as backend API, supporting multiple languages and minority groups stay the same during the extension. 


% With some efforts in the customization of crawlers and wording, formatting in the frontend, this dashboard can be easily adapted to other crisis for keeping the public informed with the latest status and calming them down.
% As we can adopt the free infrastructure like GitHub Action\footnote{\url{https://github.com/features/actions}} for hosting the project, OpenStreetMap\footnote{\url{https://www.openstreetmap.org/}} for visualizing spatial information, the initial cost of development of this dashboard is also minimized.

% \subsection{Implication about the Education}
% Most team members of this social-good project are an ongoing bachelor or postgraduate students from different education backgrounds. 
% Different from assignments in the university, our project is targeting real users to solve a real-world problem. 
% Participating in this project is a great learning process for them.
% Since there are thousands of users of this dashboard with a tremendous social impact, students are well motivated to sharpe their expertise and absorb the new knowledge during the project.
% %As most of the members in our volunteer group are still on campus, students majored in Computer Science or Business. Being participated in this project is also a learning process for them. Students are divided into different groups based on their backgrounds. 
% For example, Computer Science students are in charge of the data team and the development team with learning how to write and use a crawler to collect and aggregate data from different sources.
% They also learn not only the basic React JS coding, but also the CI/CD process, the collaboration on version control system (VCS), UI/UX designs, and software testing.
% Students from the business school use the knowledge learned from courses to try different promotion strategies, analyzing users' behavior, creating promotion posters and engaging with end users.

% %, whereas students from the business school are in the communication team. The data team learns how to write and use a crawler to collect data from different sources and use code to modify data format. The development team learns not only the basic React JS coding, but also the CI/CD process, the Github collaboration, UI/UX designs, and etc. And for the communication team, they use the knowledge learned from courses to promote the website, build up graphics, manage different social media accounts, and communicate with public users. The three teams also learn to figure out an efficient way to communicate and collaborate.

% Apart from reshaping individual expertise, this project also provides an opportunity for them to learn the collaboration within a big team.
% They have to collaborate well within and across three teams including data, development and communication groups.
% We received a great number of positive feedbacks from our team members about their learning experience in this project such as

% \say{\textit{It has been wonderful to work with such a motivated, extremely knowledgeable team. Most of my previous projects were individual, but everyone has been extremely encouraging, and have been very fortunate to have the opportunity to work with people of such a wide range of skills and backgrounds.}} 

% \say{\textit{It is such a pleasure to be able to contribute to something meaningful, and I am feeling proud of being part of the team.}}, 

% \say{\textit{This whole experience has been worthwhile, and I hope to contribute to similar endeavours going forward throughout my postgraduate studies.}}
% %Different from assignments in the university, our project is targeting real users to solve a real-world problem. A lot of the group members told us that this project is an opportunity to practice what they learned from the university and making some meaning contribution to the world. They also hope to have another opportunity in the future. We select some of their feedback as examples: \say{\textit{It has been wonderful to work with such a motivated, extremely knowledgeable team. Most of my previous projects were individual, but everyone has been extremely encouraging, and have been very fortunate to have the opportunity to work with people of such a wide range of skills and backgrounds.}}, \say{\textit{It is such a pleasure to be able to contribute to something meaningful, and I am feeling proud of being part of the team.}}, \say{\textit{This whole experience has been worthwhile, and I hope to contribute to similar endeavours going forward throughout my postgraduate studies.}}

\chen{may write some implication of this work to other related research. You can still separate it to three parts i.e., research, development and education.}



==> pattern.tex <==
\section{Patterns During the development}
\label{sec:pattern}
\chen{Please remove the patterns and put the content into positive lessons and negative lessons. For negative lessons, can we make it more abstract so called ``pitfalls''?}

\textbf{Pattern 1: Flat organization}
%Form Team: agile recruiting/ team / discussion / flat organisation
A flat organization is an organization which has few levels of management between management and staff. 

The group adopted a flat organization model that consists of 2 tiers to gain creativity and productivity among the 200 volunteer contributors. 

The first tier is the standing members of approximately thirty core people who communicate with PM regularly. Four functional teams were formed among these people, including Development, Data, News, and Promotion. These functional teams work collaboratively in the software life cycle. A typical operation example is that Promotion team get feedback from the users and address it to the group. The Development team then work out an improvement or new feature plan. Then the Data team model and collect data while it is being implemented. Finally, the Promotion team will communicate the new change to the users and collect feedback.

The second tier is broad contributors. When the functional teams are working on a task, they have autonomy at all stages. They could call for meetings to get contributors involved in the decision making, such as the design of a new feature, the improvement of existing functionalities, or the human resource plan. When it is needed, they could recruit from these contributors, or even form new teams to share workload or work in parallel.

Such structure empowered the organization to react to the requirement of the users promptly, which leads to a rapidly evolving product. Furthermore, because the members are well informed about the contextual information, their enthusiasm for the project maintained longer.

-----
1. What is this pattern. Why did we use this pattern. Explain the advantage with an example.


different teams, how do they collaborate
2. volunteer nature
3. flat 
4. creativity

\textbf{Pattern 2: Monitor the Expanding Cost}
%web development
A nonprofit online project can be costly, even when human resource cost, office space cost, overhead cost and software licensing cost are zero. 

The group bears no cost during the development of Minimum Viable Product, but it changed soon after the product is online. They chose to use a commercial map API which is free up to 50000 loads per month. The traffic volume was underestimated. After the product is online, it soon exceeded the free quotation and started to build up a bill which was unbearable for them.

Then the team worked several ways to solve the problem. They first switched temporarily to a free substitute. Though it compromised their core functionality, it prevented the bill from increasing. Then they negotiated with the commercial map API vendor for a discount. Due to the nonprofit nature of the project, the group gained a 3-month free usage concession.

Similar situations happened to other SAAS the group was using such as Slack and AWS.

\textbf{Pattern 3: Start with small and experienced team and expand as needed}
A group of small teams of highly competent people is the best way to maintain productivity as well as reducing communication overhead and decision-making cost. The size of a group can be easily expanded in the context of volunteering, but it is essential to resist the temptation to put every volunteer available into the project. 
The group learnt this the hard way. When trying to implement automatic data collecting software, the team started with eight people but only achieved less than 20 percent of all the deliverables in three weeks. Then an experienced team member took over the job, spent a week and finished the whole system. Now it is working smoothly. 
There are many reasons for this. From one hand, it takes time for people added to a project to become familiar with the contextual information to be ready to generate value. So communication efficiency decreases as the number of people increases. From another hand, software development tasks are often not divisible, which means the added people will not be able to work in parallel to increase efficiency. 

\textbf{Pattern 4: Develop only what is needed now}
Developers were trained to be farsighted, to design software that has excellent extensibilities. However, in practice, it is keen to know that the software will always evolve in response to the rapidly changing reality.

In the dashboard project, their data collection team soon realised an issue: the data sources they are delaying on often change the structure of their data. Data attributes often change got their names changed, reformatted, or even become unavailable. The data model and website code often break, which caused much work.

The team tried to make the application more extensible for the changes to try to provide a robust code once and for all, but it never worked. In one version, they worked out a perfect library to collect data from a state government's website that can handle all kind of changes within the HTML document, but the state government changed to use PowerBI which is another entirely different way to display the data, thus causing the total failure of the function again. The team soon got frustrated with this sort of coding.

Then the team changed their way. They arranged shifts to monitor changes of the data source, and work on quick and simple code exactly for the change. This strategy not only reduced the development time and unnecessary code but also increased the sense of satisfaction of the developers. 


\textbf{Pattern 5: Choose Scalable Technologies} "When a technology is scalable, it is flexible, efficient and handy to program. It
also adapts well to a scaled use of the product."\cite{dande2014software} Technology stack need to be chosen wisely. When deciding which technology will be used for the project, developers tend to choose the one that they are familiar with, which saves their "study efforts". However, this may not be the most suitable technology for the project. As most of the products need to be updated quite frequent\cite{}, no matter it's a simple upgrade or a new feature, a non-scalable technology may cost even more time to implement or in the worst case you'll have to switch to a new technology. 

Though time is limited for volunteer groups like us or startups, it's still worth to spend time on choosing scalable technologies at the design phase. Don't just simply pick the one the team has experience with, also need to ask the whole develop team to analyze the alternatives see which one fits the current scenario and the future designs to avoid further lost.
% Han

\textbf{Pattern 6: Design and conduct experiments to find out about user preferences}\cite{dande2014software} When making UI/UX decisions, it's always important for the team to think about user preferences. Because the develop team are not the users who will actually use it, user group in the most of time can be a lot different with develop group in terms of background, age, etc. 

A simple way would be having a bunch of testing users, who is willing to provide their opinions to the develop team, and conduct a A/B test\cite{} to them before you want to release something new. Another way could be release the initial design at early age, then asking feedback from users to improve the design. The alternative is a bit risk though, as the a lot of the users are lazy for leaving feedback, they may just leave and never come back. So it suits those project who already have a number of solid users and willing to take risks.

% Han

\textbf{Pattern 7: Use tools to collect data about user behavior}\cite{dande2014software} As discussed above, it's important to understand user preferences. Instead of conducting user experiments, analyze user behavior on your product can also be helpful with understanding user preference. For example, knowing which part of your project is being visited mostly, or in which sequence users normally visit could indicate users preference and their usage patterns so that in the future you can add these knowledge as factors into the design and development phases or improve current features.

Some commonly used tools for apps and websites are like Google Analytics\footnote{\url{https://analytics.google.com/}}, Heap\footnote{\url{https://heap.io/}}. They are designed to be easy embedded into your project and offering more than simple user behavior analysis. For instance, in our practice, we noticed that the default language of the accessing devices varies from en, to zh, ja, ko and so on. So we realized that a lot of our users don't have English as their primary language, and we produced the multi language version based on the Anaytics Report which have received some positive feedback from users. 
% Han

\textbf{Pattern 8: Create the development culture before processes}\cite{dande2014software} The development culture here is like a general guide book of the startup or a volunteer group. It tells the value of the group and set some basic consensus in terms of the overall goal, approaches and activities. As a non-commercial volunteer group like us, most of our people work on interest-driven and they may just leave the group when losing interests and on the opposite new volunteers are also being expected at anytime. So instead of some solid  processes, we want to create a flexible but diverse environment at the very beginning. For example, similar to an Open source management concept \cite{}, we have a to-do checklist and let developers pick tasks freely. But we also have adopted Agile management \cite{}, to have retrospective meetings with core development team for summarizing works and set up goals and tasks. And most of the team members feel satisfied with this pattern.
% Han

\textbf{Pattern 9: Use the most efficient programming languages and platforms} \cite{dande2014software} Time is limited at the beginning phase. Use the most efficient programming languages and platforms can help you quickly deploy your project and take the lead in the business competition. 
% Han


\textbf{Pattern 10: Make features easy to remove} \cite{dande2014software} As the project grows, you may face many upgrades to the existed project. Sometimes when it's too hard to change, you may need to remove the whole thing and rewrite from scratch. So when creating a new component of the project, make sure to modularize the project and prepare for the future changes.


